Towards a debuggable kernel design

This paper describes what it means for a kernel to be debuggable and proposes a kernel design with debuggability in mind. We evaluate the proposed kernel design by comparing the iterations required in cyclic debugging for different classes of bugs in a vanilla monolithic kernel to a variant enhanced with our design rules for debuggability. We discuss the trade offs involved in designing a debuggable kernel.

==> ExcOverhead.tex <==
\begin{figure*}
\label{fig:b1}
\caption{Execution Overhead for d-Pebbles}
\end{figure*}
